Measurement of the transverse momentum and $\phi^*_{\eta}$ distributions of Drell-Yan lepton pairs in proton-proton collisions at $\sqrt{s}=8$ TeV with the ATLAS detector

Distributions of transverse momentum $p_T^{ll}$ and the angular variable $\phi^*_\eta$ of Drell--Yan lepton pairs are measured in 20.3 fb$^{-1}$ of proton--proton collisions at $\sqrt{s}=8$ TeV with the ATLAS detector at the LHC. Measurements in electron-pair and muon-pair final states are corrected for detector effects and combined. Compared to previous measurements in proton--proton collisions at $\sqrt{s}=7$ TeV, these new measurements benefit from a larger data sample and improved control of systematic uncertainties. Measurements are performed in bins of lepton-pair mass above, around and below the Z-boson mass peak. The data are compared to predictions from perturbative and resummed QCD calculations. For values of $\phi^*_\eta < 1$ the predictions from the Monte Carlo generator ResBos are generally consistent with the data within the theoretical uncertainties. However, at larger values of $\phi^*_\eta$ this is not generally the case. Monte Carlo generators based on the parton-shower approach are unable to describe the data over the full range of $p_T^{ll}$ and the fixed-order prediction of DYNNLO falls below the data at high values of $p_T^{ll}$. ResBos and the parton-shower Monte Carlo generators provide a much better description of the evolution of the $\phi^*_\eta$ and $p_T^{ll}$ distributions as a function of lepton-pair mass and rapidity.

==> tables/ZPtLowM1Val.tex <==
\begin{table*}
\centering
\caption{The values of $(1/\sigma)\,d\sigma/d\Zpt$ in each bin of \Zpt\ for the electron and muon channels separately (for various truth level definitions) and for the Born level combination in the kinematic region $ 12 \textrm{ GeV} \leq M_{\ell\ell} <  20 \textrm{ GeV},\ 0.0 \leq |y_{\ell\ell}| < 2.4$. The associated statistical and systematic (both uncorrelated and correlated between bins) are provided in percentage form.}
\resizebox{\textwidth}{!}{
\centering 
\begin{tabular}{ c  cccccc } \toprule  
 Bin & \multicolumn{6}{c}{$(1/\sigma)\,d\sigma/d\Zpt$ $\pm$ Statistical [\%] $\pm$ Uncorrelated systematic [\%] $\pm$ Correlated systematic [\%] } \\ 
 \cmidrule(r){2-7} 
  & 	\multicolumn{2}{c}{Electron channel} & \multicolumn{3}{c}{Muon channel} & Combination \\ 
 \cmidrule(r){2-3} \cmidrule(r){4-6} \cmidrule(r){7-7}
  & Dressed & Born & Bare & Dressed & Born & Born \\ 
 45.0 -- 55.0 &2.574e-02 $\pm$  1.9 $\pm$  1.4$\pm$   2.3&2.573e-02 $\pm$  1.9 $\pm$  1.4$\pm$   2.3&2.794e-02 $\pm$  1.3 $\pm$  0.3$\pm$   0.7&2.788e-02 &2.780e-02 $\pm$  1.3 $\pm$  0.3$\pm$   1.3&2.740e-02 $\pm$  1.1 $\pm$  0.4$\pm$   1.1 \\ 
 55.0 -- 65.0 &2.194e-02 $\pm$  2.3 $\pm$  1.6$\pm$   1.7&2.198e-02 $\pm$  2.3 $\pm$  1.6$\pm$   1.8&2.179e-02 $\pm$  1.6 $\pm$  0.5$\pm$   0.5&2.169e-02 &2.171e-02 $\pm$  1.6 $\pm$  0.5$\pm$   0.7&2.177e-02 $\pm$  1.3 $\pm$  0.5$\pm$   0.8 \\ 
 65.0 -- 75.0 &1.540e-02 $\pm$  2.6 $\pm$  2.7$\pm$   2.9&1.541e-02 $\pm$  2.6 $\pm$  2.7$\pm$   2.9&1.536e-02 $\pm$  1.9 $\pm$  0.5$\pm$   0.6&1.534e-02 &1.539e-02 $\pm$  1.9 $\pm$  0.5$\pm$   1.3&1.535e-02 $\pm$  1.6 $\pm$  0.7$\pm$   1.2 \\ 
 75.0 -- 85.0 &1.035e-02 $\pm$  3.2 $\pm$  1.4$\pm$   1.9&1.034e-02 $\pm$  3.2 $\pm$  1.4$\pm$   2.2&1.037e-02 $\pm$  2.3 $\pm$  0.7$\pm$   1.1&1.041e-02 &1.044e-02 $\pm$  2.3 $\pm$  0.7$\pm$   1.1&1.036e-02 $\pm$  1.9 $\pm$  0.7$\pm$   1.1 \\ 
 85.0 -- 105.0 &6.310e-03 $\pm$  2.5 $\pm$  1.1$\pm$   2.0&6.327e-03 $\pm$  2.5 $\pm$  1.1$\pm$   2.1&5.971e-03 $\pm$  2.1 $\pm$  0.6$\pm$   1.1&5.987e-03 &5.987e-03 $\pm$  2.1 $\pm$  0.6$\pm$   1.4&6.061e-03 $\pm$  1.6 $\pm$  0.6$\pm$   1.3 \\ 
 105.0 -- 150.0 &2.174e-03 $\pm$  2.7 $\pm$  1.0$\pm$   2.2&2.164e-03 $\pm$  2.7 $\pm$  1.0$\pm$   2.3&2.021e-03 $\pm$  2.4 $\pm$  0.7$\pm$   1.4&2.037e-03 &2.040e-03 $\pm$  2.4 $\pm$  0.7$\pm$   1.4&2.065e-03 $\pm$  1.8 $\pm$  0.6$\pm$   1.3 \\ 
 150.0 -- 200.0 &5.582e-04 $\pm$  4.7 $\pm$  1.9$\pm$   3.4&5.565e-04 $\pm$  4.7 $\pm$  1.9$\pm$   3.6&4.883e-04 $\pm$  4.6 $\pm$  1.7$\pm$   2.5&4.950e-04 &4.906e-04 $\pm$  4.6 $\pm$  1.7$\pm$   2.6&5.114e-04 $\pm$  3.3 $\pm$  1.2$\pm$   2.3 \\ 
 200.0 -- 900.0 &1.961e-05 $\pm$  9.6 $\pm$  2.9$\pm$   4.6&1.953e-05 $\pm$  9.6 $\pm$  2.9$\pm$   4.9&1.524e-05 $\pm$  7.1 $\pm$  1.9$\pm$   3.4&1.518e-05 &1.505e-05 $\pm$  7.1 $\pm$  1.9$\pm$   4.3&1.619e-05 $\pm$  5.7 $\pm$  1.6$\pm$   3.5 \\ 
\bottomrule 
\end{tabular}
}
\label{tab:CombZPtLowM1}
\end{table*}


==> tables/ZPtLowM2Val.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\centering 
\begin{tabular}{ c  cccccc } \toprule  
 Bin & \multicolumn{6}{c}{$(1/\sigma)\,d\sigma/d\Zpt$ $\pm$ Statistical [\%] $\pm$ Uncorrelated systematic [\%] $\pm$ Correlated systematic [\%] } \\ 
 \cmidrule(r){2-7} 
  & 	\multicolumn{2}{c}{Electron channel} & \multicolumn{3}{c}{Muon channel} & Combination \\ 
 \cmidrule(r){2-3} \cmidrule(r){4-6} \cmidrule(r){7-7}
  & Dressed & Born & Bare & Dressed & Born & Born \\ 
 45.0 -- 55.0 &2.303e-02 $\pm$  2.3 $\pm$  0.9$\pm$   2.2&2.292e-02 $\pm$  2.3 $\pm$  0.9$\pm$   2.3&2.306e-02 $\pm$  1.6 $\pm$  0.6$\pm$   1.1&2.297e-02 &2.287e-02 $\pm$  1.6 $\pm$  0.6$\pm$   1.7&2.272e-02 $\pm$  1.3 $\pm$  0.5$\pm$   1.4 \\ 
 55.0 -- 65.0 &1.746e-02 $\pm$  2.7 $\pm$  1.4$\pm$   1.8&1.754e-02 $\pm$  2.7 $\pm$  1.4$\pm$   1.8&1.759e-02 $\pm$  2.0 $\pm$  0.7$\pm$   0.9&1.758e-02 &1.771e-02 $\pm$  2.0 $\pm$  0.7$\pm$   1.0&1.760e-02 $\pm$  1.6 $\pm$  0.7$\pm$   1.0 \\ 
 65.0 -- 75.0 &1.215e-02 $\pm$  3.2 $\pm$  1.3$\pm$   2.3&1.225e-02 $\pm$  3.2 $\pm$  1.3$\pm$   2.3&1.229e-02 $\pm$  2.4 $\pm$  1.0$\pm$   1.5&1.233e-02 &1.243e-02 $\pm$  2.4 $\pm$  1.0$\pm$   1.7&1.227e-02 $\pm$  1.9 $\pm$  0.8$\pm$   1.4 \\ 
 75.0 -- 85.0 &8.630e-03 $\pm$  3.7 $\pm$  1.7$\pm$   3.1&8.693e-03 $\pm$  3.7 $\pm$  1.7$\pm$   3.1&8.436e-03 $\pm$  2.9 $\pm$  1.3$\pm$   2.0&8.416e-03 &8.439e-03 $\pm$  2.9 $\pm$  1.3$\pm$   2.1&8.462e-03 $\pm$  2.3 $\pm$  1.0$\pm$   1.8 \\ 
 85.0 -- 105.0 &5.133e-03 $\pm$  3.1 $\pm$  1.4$\pm$   3.3&5.179e-03 $\pm$  3.1 $\pm$  1.4$\pm$   3.4&5.167e-03 $\pm$  2.5 $\pm$  1.2$\pm$   1.9&5.179e-03 &5.226e-03 $\pm$  2.5 $\pm$  1.2$\pm$   1.9&5.157e-03 $\pm$  2.0 $\pm$  0.9$\pm$   1.9 \\ 
 105.0 -- 150.0 &1.856e-03 $\pm$  3.1 $\pm$  1.4$\pm$   3.9&1.869e-03 $\pm$  3.1 $\pm$  1.4$\pm$   4.0&1.803e-03 $\pm$  2.6 $\pm$  1.0$\pm$   2.1&1.821e-03 &1.828e-03 $\pm$  2.6 $\pm$  1.0$\pm$   2.3&1.818e-03 $\pm$  2.0 $\pm$  0.8$\pm$   2.2 \\ 
 150.0 -- 200.0 &4.994e-04 $\pm$  5.1 $\pm$  2.4$\pm$   4.8&5.030e-04 $\pm$  5.1 $\pm$  2.4$\pm$   5.1&4.198e-04 $\pm$  5.3 $\pm$  2.3$\pm$   3.2&4.229e-04 &4.229e-04 $\pm$  5.3 $\pm$  2.3$\pm$   3.3&4.539e-04 $\pm$  3.7 $\pm$  1.6$\pm$   2.9 \\ 
 200.0 -- 900.0 &1.830e-05 $\pm$  6.8 $\pm$  2.8$\pm$   5.4&1.828e-05 $\pm$  6.8 $\pm$  2.8$\pm$   6.4&1.580e-05 $\pm$  7.0 $\pm$  2.7$\pm$   3.4&1.604e-05 &1.597e-05 $\pm$  7.0 $\pm$  2.7$\pm$   3.6&1.666e-05 $\pm$  5.0 $\pm$  1.9$\pm$   3.6 \\ 
\bottomrule 
\end{tabular}
}
\caption{The values of $(1/\sigma)\,d\sigma/d\Zpt$ in each bin of \Zpt\ for the electron and muon channels separately (for various truth level definitions) and for the Born level combination in the kinematic region $ 20 \textrm{ GeV} \leq M_{\ell\ell} <  30 \textrm{ GeV},\ 0.0 \leq |y_{\ell\ell}| < 2.4$. The associated statistical and systematic (both uncorrelated and correlated between bins) are provided in percentage form.}\label{tab:CombZPtLowM2}
\end{table*}


==> tables/ZPtLowM3Val.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\centering 
\begin{tabular}{ c  cccccc } \toprule  
 Bin & \multicolumn{6}{c}{$(1/\sigma)\,d\sigma/d\Zpt$ $\pm$ Statistical [\%] $\pm$ Uncorrelated systematic [\%] $\pm$ Correlated systematic [\%] } \\ 
 \cmidrule(r){2-7} 
  & 	\multicolumn{2}{c}{Electron channel} & \multicolumn{3}{c}{Muon channel} & Combination \\ 
 \cmidrule(r){2-3} \cmidrule(r){4-6} \cmidrule(r){7-7}
  & Dressed & Born & Bare & Dressed & Born & Born \\ 
 45.0 -- 55.0 &2.193e-02 $\pm$  2.3 $\pm$  0.7$\pm$   1.7&2.193e-02 $\pm$  2.3 $\pm$  0.7$\pm$   1.8&2.255e-02 $\pm$  1.7 $\pm$  0.5$\pm$   1.0&2.261e-02 &2.255e-02 $\pm$  1.7 $\pm$  0.5$\pm$   1.2&2.237e-02 $\pm$  1.3 $\pm$  0.4$\pm$   1.1 \\ 
 55.0 -- 65.0 &1.610e-02 $\pm$  2.7 $\pm$  1.4$\pm$   1.4&1.628e-02 $\pm$  2.7 $\pm$  1.4$\pm$   1.6&1.605e-02 $\pm$  2.1 $\pm$  0.8$\pm$   1.0&1.603e-02 &1.621e-02 $\pm$  2.1 $\pm$  0.8$\pm$   1.4&1.627e-02 $\pm$  1.6 $\pm$  0.7$\pm$   1.1 \\ 
 65.0 -- 75.0 &1.131e-02 $\pm$  3.2 $\pm$  1.1$\pm$   1.6&1.151e-02 $\pm$  3.2 $\pm$  1.1$\pm$   1.6&1.070e-02 $\pm$  2.7 $\pm$  1.1$\pm$   1.3&1.065e-02 &1.076e-02 $\pm$  2.7 $\pm$  1.1$\pm$   1.3&1.104e-02 $\pm$  2.1 $\pm$  0.8$\pm$   1.0 \\ 
 75.0 -- 85.0 &7.101e-03 $\pm$  4.2 $\pm$  1.5$\pm$   2.3&7.197e-03 $\pm$  4.2 $\pm$  1.5$\pm$   2.5&7.567e-03 $\pm$  3.2 $\pm$  1.2$\pm$   1.6&7.513e-03 &7.605e-03 $\pm$  3.2 $\pm$  1.2$\pm$   2.1&7.474e-03 $\pm$  2.6 $\pm$  0.9$\pm$   1.8 \\ 
 85.0 -- 105.0 &4.393e-03 $\pm$  3.5 $\pm$  1.4$\pm$   2.5&4.453e-03 $\pm$  3.5 $\pm$  1.4$\pm$   2.5&4.381e-03 $\pm$  2.8 $\pm$  1.2$\pm$   1.8&4.408e-03 &4.464e-03 $\pm$  2.8 $\pm$  1.2$\pm$   1.8&4.455e-03 $\pm$  2.2 $\pm$  0.9$\pm$   1.5 \\ 
 105.0 -- 150.0 &1.602e-03 $\pm$  3.3 $\pm$  1.5$\pm$   2.9&1.622e-03 $\pm$  3.3 $\pm$  1.5$\pm$   3.0&1.535e-03 $\pm$  3.2 $\pm$  1.1$\pm$   2.4&1.546e-03 &1.566e-03 $\pm$  3.2 $\pm$  1.1$\pm$   2.4&1.590e-03 $\pm$  2.3 $\pm$  0.9$\pm$   1.9 \\ 
 150.0 -- 200.0 &4.198e-04 $\pm$  5.6 $\pm$  1.8$\pm$   3.6&4.231e-04 $\pm$  5.6 $\pm$  1.8$\pm$   3.8&4.510e-04 $\pm$  5.3 $\pm$  2.3$\pm$   4.3&4.514e-04 &4.520e-04 $\pm$  5.3 $\pm$  2.3$\pm$   4.3&4.383e-04 $\pm$  3.8 $\pm$  1.4$\pm$   3.1 \\ 
 200.0 -- 900.0 &1.649e-05 $\pm$  7.4 $\pm$  5.1$\pm$   6.0&1.694e-05 $\pm$  7.4 $\pm$  5.1$\pm$   6.2&1.434e-05 $\pm$  7.4 $\pm$  3.4$\pm$   7.4&1.467e-05 &1.486e-05 $\pm$  7.4 $\pm$  3.4$\pm$   7.7&1.587e-05 $\pm$  5.3 $\pm$  2.9$\pm$   5.3 \\ 
\bottomrule 
\end{tabular}
}
\caption{The values of $(1/\sigma)\,d\sigma/d\Zpt$ in each bin of \Zpt\ for the electron and muon channels separately (for various truth level definitions) and for the Born level combination in the kinematic region $ 30 \textrm{ GeV} \leq M_{\ell\ell} <  46 \textrm{ GeV},\ 0.0 \leq |y_{\ell\ell}| < 2.4$. The associated statistical and systematic (both uncorrelated and correlated between bins) are provided in percentage form.}\label{tab:CombZPtLowM3}
\end{table*}

